Exploring with Sticky Mittens: Reinforcement Learning with Expert Interventions via Option Templates

Long horizon robot learning tasks with sparse rewards pose a significant challenge for current reinforcement learning algorithms. A key feature enabling humans to learn challenging control tasks is that they often receive expert intervention that enables them to understand the high-level structure of the task before mastering low-level control actions. We propose a framework for leveraging expert intervention to solve long-horizon reinforcement learning tasks. We consider \emph{option templates}, which are specifications encoding a potential option that can be trained using reinforcement learning. We formulate expert intervention as allowing the agent to execute option templates before learning an implementation. This enables them to use an option, before committing costly resources to learning it. We evaluate our approach on three challenging reinforcement learning problems, showing that it outperforms state-of-the-art approaches by two orders of magnitude. Videos of trained agents and our code can be found at: https://sites.google.com/view/stickymittens

==> background.tex <==
\section{Background}

We consider the RL setting where an agent interacts with an environment modeled as an MDP \citep{sutton2018reinforcement}.


\begin{definition}[\textbf{MDP}]
\label{def:mdp}
A \emph{Markov Decision Process (MDP)} is a tuple $\env=(\mathcal{S}, \mathcal{A}, \mathcal{P}, \mathcal{R}, \gamma, \init )$, where  $\mathcal{S} \subseteq \reals^n$ is the set of states, $\mathcal{A} \subseteq \reals^m$ is the set of actions, $\mathcal{P}(s'|s,a)$ is the probability of transitioning from state $s$ to $s'$ upon taking action $a$, $\mathcal{R}(s,a)$ is the reward accrued in state $s$ upon taking action $a$, $\gamma \in [0,1)$ is the discount factor, and $\init$ is the initial state distribution.
\end{definition}

The dynamics evolve over discrete time steps, where the agent transitions from state $s_t$ to $s_{t+1}\sim\mathcal{P}(\cdot|s_t,a_t)$ by taking an action $a_t$, receiving a reward $r_t=\mathcal{R}(s_t,a_t)$.  
The \emph{return} at time $t$ from state $s_t$ is the sum of discounted future rewards $\mathbf{R}(s_t) = \sum_{j=t}^{\infty} \gamma^{j-t}r(s_j,a_j)$. A deterministic policy $\pi$ is a mapping $\pi : \mathcal{S} \rightarrow \mathcal{A}$; given $\pi$, the agent executes action $a = \pi(s)$ in state $s$. The value of a state for policy $\pi$ is the expected return $\mathbf{R}_\pi(s_0)$ starting from state $s_0$, while executing the policy $\pi$ at every step, $a_t = \pi(s_t)$. 
The optimal policy $\pi^*$ maximizes the reward starting from the initial state distribution---i.e., $ \pi^* = \argmax  V^{\init}(\pi)$,
where 
$V^{\init}(\pi) = \mathbb{E}_{s_0 \in \init} [\mathbf{R}_\pi(s_0)]$. The goal is to learn $\pi^*$.
\begin{wrapfigure}{r}{0.3\textwidth}
\begin{center}
\includegraphics[width=4cm, height=2cm]{Figures/option_template_h.png}
\end{center}
\caption{Option vs Option Template.}
\label{fig:uber_actions}
\end{wrapfigure}
Semi-MDPs (SMDPs) extend this framework by allowing temporally extended actions---i.e., policies executed over multiple steps---called \emph{options}~\citep{options_paper}.
\begin{definition}[\textbf{Option}]
\label{defn:option}
An \emph{option} $o$ is a tuple $o :=(\optionI, \optionT, \pi)$, 
where $\optionI \subseteq S$ is its set of  initial states, $\optionT: \mathcal{S} \rightarrow [0,1]$ is a termination condition, and $\pi: \mathcal{S} \rightarrow \mathcal{A}$ is a policy.
\end{definition}
For now, assume that we have a set $\optionO$ of options available for an MDP. Intuitively, options constrain the search space over policies, thereby guiding exploration performed by the agent towards more promising action sequences. In particular, we now consider policies $\Pi:\mathcal{S}\to\optionO$ that map a state $s\in\optionI$ (i.e., $s$ is a valid initial state for $o$) to an option $o=\Pi(s)$. Then, the agent uses policy $\pi$ until the termination condition holds. More precisely, after taking action $a=\pi(s)$ and transitioning to state $s'\sim\mathcal{P}(\cdot|s,a)$, it stops using $\pi$ with probability $\optionT(s_{t+1})$ and chooses another option $o'=\Pi(s')$; otherwise, it continues using $\pi$.


For Markovian options, the termination condition $\optionT$ or the option sub-policy $\pi$ depends only on the current state only. In practice, it is useful to have the ability to \textit{time out}, i.e., to terminate an option even if it does not satisfy some desirable end goal. Suppose that an option $o$ is invoked at time $t$ in state $s_t$, and assume that under the control of this option, the system follows a $k$ step trajectory $ \mathsf{Tr}^{o}(s_t, k)=(s_{t}, a_{t}, r_{t}, s_{t+1}, \dots , s_{t+k})$.
It is possible that for $t \leq i < t + k$, the action $a_i$ depends on the entire history $\mathsf{Tr}^{o}(s_t, i)$ from $t$ until $t + i$.  This use of memory renders the behavior non-Markovian. Denoting the set of all such state-action trajectories as $H$, we can allow option policies $\pi: H \rightarrow \mathcal{A}$, and termination conditions $\optionT: H \rightarrow [0,1]$ to be semi-Markovian. Now, we recall the definition of Semi-MDPs as an extension of MDPs:

\begin{definition}[\textbf{Semi-MDP},  \citet{options_paper}]
A semi-MDP is a tuple $(\mathcal{S}, \mathcal{O}, \mathcal{P}, \mathcal{R}, \gamma, \init )$, where $\mathcal{S}$ is a set of states, $\mathcal{O}$ is a set of semi-Markovian options, $\mathcal{P}$ is the transition probability between states, $\mathcal{R}$ is the reward function, $\gamma \in [0,1)$ is the discount factor, and $\init$ is the initial state distribution.
\end{definition}

The state-prediction part of the model for taking an option $o$, in state $s \in \optionI $ and transitioning to $s'$, is given by \citet{options_paper}: $ P(s'| s, o) = \sum_{k=1}^{\infty} \gamma^k p(s',s,k)$, 
where $p(s',s,k)$ is the probability that the option terminates in $s'$ after $k$ steps from the time the option is invoked. Let $\mathscr{E}(o,s,t)$ be the event of taking an option $o$ while in state $s$ at time $t$. Then the time-discounted reward is $ \mathbf{R}(s, o) = \mathbb{E}\{r_{t} + \gamma r_{t+1} + \dots + \gamma^k r_{t+k} | \mathscr{E}(o,s,t) \} $,
where $t+k$ is the random time at which the option $o$ terminates. 
The option-value form of standard value iteration is, for $s \in \mathcal{S}$ and $o \in \mathcal{O}$, \citep[][eq. 12]{options_paper},
\citep{Barto03recentadvances}
\begin{equation}
    \label{eq:option-value}
    Q^{*}_{\optionO}(s, o) = R(s, o) + \sum_{s' \in S}P(s'|s, o) \max_{o' \in \optionO} Q^*_{\optionO}(s', o'),
\end{equation}
where $s'$ is the state the system reaches after executing option $o$ starting from state $s$. SMDP value learning updates the $Q$-values at the end of each option termination as  \citep[][p. 195]{options_paper}:
\begin{equation}
    \label{eq:value-update}
    Q^{i+1}(s, o) \leftarrow Q^i(s, o) + \alpha[r_c + \gamma^k \max_{o' \in \optionO }Q^i(s', o') - Q^i(s, o)],
\end{equation}
for similar definitions of $k$, $s$, $s'$, with $r_c$ being the cumulative discounted reward over the time horizon, and $\alpha \in (0,1)$ the learning rate. 
Choosing a function approximator parameterized by $\theta$ to represent $Q(s, o; \theta)$, with a loss given by :  
$L(\theta_i) = [r + \gamma^k \max_{o' \in O}Q^i(s', o';\theta_i) - Q^i(s, o; \theta_i)]^2$,
allows one to use standard Q-learning \citep{deep-q-paper} methods to train with options.



==> introduction_CoRL_small.tex <==
Reinforcement learning is an effective tool to solve difficult tasks such as robot planning and locomotion~\citep{demo_RL}. In order to apply RL effectively to practical applications with a high-dimensional state and action space, exploration is a challenge. Generally, complex sequences of actions are required to achieve any nonzero reward. Hence, random exploration will take extremely long to find a nonzero reward signal. 

\emph{Options} are an RL tool to circumvent this problem~\citep{options_paper}. Options are policies designed to achieve intermediate subgoals. 
% For instance, in robot grasping tasks, an option might enable the robot to grasp a block, which is a subgoal needed to build a tower out of blocks. Then, the goal becomes to learn a policy mapping each state to an option, instead of a concrete action to take.  
Options naturally guide exploration, making it more likely that the agent encounters nonzero rewards.

When learning to perform complex visual-motor skills, humans often rely on expert interventions to help them escape these challenging reward plateaus. For instance, the \textit{sticky-mittens} experiment~\citep{sticky_mittens_exp} considers children who have not yet learned to grasp objects. They give a subset of these children mittens covered with Velcro hooks and allow them to play with toys fitted with Velcro loops, making it significantly easier for them to grasp these toys. Even if the Velcro is taken away, these children learn how to grasp objects significantly faster than children not exposed to this experience. In other words, enabling children to explore unreachable parts of the state space helps guide them towards skills that are worth learning. 
%This extends beyond fine motor skills and is a well known phenomenon in developmental psychology.
This is a well known phenomenon in developmental psychology, which extends beyond fine motor skills.

In this paper, we design an RL algorithm based on the idea from the sticky-mittens experiment of providing training time expert help. In particular, our algorithm provides the agent with an alternative Markov Decision Process (MDP) where the agent can leap multiple states without first learning a policy to do so in the original MDP. We term such a jumping mechanism an \emph{option template}. Option templates are described using a set of initial states and a set of final states.  The agent uses reinforcement learning to train an option to implement each option template. Using an option template moves the agent to a state in the desired set of final states. After this, the agent can continue exploration. As a consequence, the agent acquires the ability to use an option before deciding to spend effort to learn it. Option templates enable the agent to predict the effects of options so as to be able to plan over long and difficult tasks. % should probably stay away from the word teleport

The idea of providing external help in the learning phase is referred to as \textit{primitives} or \textit{skills} in literature. It offers a practical way to speed-up learning in a realistic setting. For instance, using parameterized action spaces for RoboCup in \citep{ICLR16-hausknecht}, stitching independent behaviors in \citep{ut_austin_robocup} and providing action primitives in \citep{action_primitives, icra22_primitves} to mention a few. 

Generally, in the more typical framework of training with options, the user is burdened with providing the agent with an implementation of each option. Thus, the agent first uses reinforcement learning to train an option to implement the specification of each option template, after which it can again use reinforcement learning to train a policy over these options. The issue with this strategy is that, in RL environments with large state spaces the options learnt need to be of a fairly generic nature, in order to be useful. Without a knowledge of the state distribution, where the options will be invoked by a higher level policy. Through the use of \emph{option templates} we decouple the implementation of an option from its utility, by providing the agent with a deterministic transition to the outcome of running the option.


% In more detail, our algorithm performs an alternating search over policies: at each iteration, it first optimizes the high-level policy over the current option templates, and then learns options to implement the option templates. It continues this iterative procedure until it has learned a policy that uses the actions in the original action space. 
Once the high-level policy learns from which states to call an option template, it provides an implicit guide to the following level. In our experiments, we demonstrate that by leveraging option templates, our algorithm can achieve an order of magnitude reduction in sample complexity compared to the typical strategy of learning the options upfront and then planning with these learned options.



\textbf{Contributions: } Our contributions are: (1) an RL algorithm that leverages option-templates, and (2) an empirical comparison with state-of-the-art RL techniques on three challenging environments, demonstrating an order-of-magnitude reduction in sample complexity.

==> introduction_through_child_development.tex <==
\section{Introduction}

In reinforcement learning (RL), the agent's goal is to maximize a reward function while exploring its environment. 
Modern techniques such as deep reinforcement learning can effectively solve this problem in large state spaces in a number of cases~\citep{deep-q-paper}, enabling reinforcement learning to solve difficult tasks such as robot planning and locomotion~\citep{demo_RL} and playing video games from visual inputs~\citep{high_dim_RL}.


In order to apply RL effectively, to practical applications with a high-dimensional state and action space, exploration is a challenge. Intuitively, in such settings, complex sequences of actions are required to achieve any nonzero reward, which means that random exploration will take extremely long to find a nonzero reward signal. Thus, learning to improve performance can be very slow.

\emph{Options} are an RL tool to circumvent this problem~\citep{options_paper}. Options are policies designed to achieve intermediate subgoals. For instance, in robot grasping tasks, an option might enable the robot to grasp a block, which is a subgoal needed to build a tower out of blocks. Then, the goal becomes to learn a policy mapping each state to an option, instead of a concrete action to take. 
Options naturally guide exploration, making it more likely that the agent encounters nonzero rewards.

When learning to perform complex visual-motor skills, humans often rely on expert interventions to help them escape these challenging reward plateaus. For instance, the \textit{sticky-mittens} experiment~\citep{sticky_mittens_exp} considers children who have not yet learned to grasp objects. They give a subset of these children mittens covered with Velcro hooks and allow them to play with toys fitted with Velcro loops, making it significantly easier for them to grasp these toys. Even if the Velcro is taken away, these children learn how to grasp objects significantly faster than children not exposed to this experience. In other words, enabling children to explore unreachable parts of the state space helps guide them towards skills that are worth learning. This extends beyond fine motor skills, and is a well known phenomenon in developmental psychology.

In this paper, we design an RL algorithm based on the idea from the sticky-mittens experiment of providing training time expert help. In particular, our algorithm provides the agent with an alternative Markov Decision Process (MDP) where the agent can leap multiple states without first learning a policy to do so in the original MDP. We term such a jumping mechanism an \emph{option template}. Option templates are described using a set of initial states and a set of final states.  The agent uses reinforcement learning to train an option to implement each option template. Using an option template teleports the agent to a state in the desired set of final states. After this, the agent can continue exploration. As a consequence, the agent acquires the ability to use an option before deciding to spend effort to learn it. 

For comparison, in the more typical framework of training with options, the user is typically burdened with providing the agent with an implementation of each option. Thus, the agent first uses reinforcement learning to train an option to implement the specification of each option template, after which it can again use reinforcement learning to train a policy over these options. The issue with this strategy is that, in RL environments with large state spaces the options learnt need to be of a fairly generic nature, in order to be useful. Without a knowledge of the state distribution, where the options will be invoked by a higher level policy. Through the use of \emph{option templates} we decouple the implementation of an option from its utility, by providing the agent with a deterministic transition to the outcome of running the option.




In more detail, our algorithm performs an alternating search over policies: at each iteration, it first optimizes the high-level policy over the current option templates, and then learns options to implement the option templates. It continues this iterative procedure until it has learned a policy that uses the actions in the original action space. 
Once the high-level policy learns from which states to call an option template, it provides an implicit guide to the following level. In our experiments, we demonstrate that by leveraging option templates, our algorithm can achieve an order of magnitude reduction in sample complexity compared to the typical strategy of learning the options upfront and then planning with these learned options.





\textbf{Contributions: } Our contributions are: (1) an RL algorithm that leverages option-templates, and (2) an empirical comparison with state-of-the-art RL techniques on three challenging environments, demonstrating an order-of-magnitude reduction in sample complexity.


==> uber_actions.tex <==
\section{Learning with Option Templates}

\subsection{Option Templates}


A key challenge with options is that it is often difficulty to supply the option policy $\pi$; while this policy can be learned, it can be hard for the agent to judge the starting state distribution.
Motivated by the sticky-mittens experiment, we consider an environment where in certain states, the agent can call a ``help switch'', called an \emph{option template}, that immediately transitions them from a state $s_t$ to a different state $s_{t+k}$; this transition captures the desired result of executing an (unimplemented) option. We denote a trajectory of this MDP starting from state $s_t$ under policy $\pi$ by $\mathsf{Tr}^{\pi}(s_t)$. 

\begin{definition}[\textbf{Option template}]
\label{defn:option_template}
An option template $a_o$ is a tuple $(\optionI, \optionT, P) $, where $\optionI \subseteq \mathcal{S}$ is a set of initial states, $\optionT: \mathcal{S} \rightarrow [0,1]$ is a termination condition, and $P$ is a distribution over states $s$ such that $\optionT(s)=1$.
\end{definition}
An option template functions like an option, by shifting control to the expert until the termination condition is reached; this termination condition $\optionT$ is intended to capture the satisfaction of some sub-goal along with a timeout mechanism. We assume the termination condition at time $t+k$ of an option template taken in state $s_t$ is of the form $\optionT(s_t, k) = \mathbf{F}_{o}(s_{t+k}) \vee (k > k^*)$, where the \emph{predicate function} $\mathbf{F}_{o}: \mathcal{S} \rightarrow \{0,1\}$ assesses visitation of some key states, and $k^*$ is an upper bound on the number of steps allowed.

Furthermore, the distribution $P$ enables us to ``teleport'' to a state that satisfies the termination condition---i.e., if an agent invokes $a_o$ from a state $s\in I$, then we sample a terminal state $s'\sim T$ and transition the MDP to $s'$.

The agent may have access to multiple option templates during training; we denote such a set (or subset) of option templates by $\mathcal{A_\optionO}$. These option templates are supplied by an expert with a knowledge of the goal. By the end of training, the agent must learn a policy to implement each option template that it uses (i.e., the final policy cannot depend on option templates). To ensure feasiblity, we assume there is an a priori unknown policy $\pi_{o}$ such that $\mathsf{Tr}^{\pi_{o}}(s_t)$ satisfies $\optionT$ (denoted as $\mathsf{Tr}^{\pi_{o}}(s_t) \models \optionT$) with probability at least $1-\delta$, for some hyperparameter $\delta \in [0,1)$. Formally, the probability of success of a given policy $\pi_o$ can be expressed as $\prob((\pi_o, \optionI, \env)\models \optionT) \ge (1-\delta)$---i.e., the trajectory starting from a state in $\optionI$ under the control of $\pi_o$ in environment $\env$ satisfies $\optionT$ with probability at least $1-\delta$. This success probability can be estimated by empirical rollouts of $ \pi_{o}$.


Next, there are different degrees of help that option templates can offer; option templates that traverse longer sequences of transitions can help the agent learn a high-level strategy more quickly since they need to make fewer decisions, but learning their implementations can be more costly. Thus, option templates can be organized in a hierarchical fashion, where longer-horizon option templates can themselves be implemented in terms of several shorter-horizon option templates.
Thus, we consider a sequence of environments $\env^0, \env^1, \dots , \env^{n-1} = \env$, equipped with option templates of varying capabilities. 

\begin{definition} [\textbf{Environment Level $\env^l$}]
An environment $\env^l$ at learning level $l$ is the original environment $\env$ with the primitive actions $\mathcal{A}$ replaced by option templates $\mathcal{A}_{\optionO}^l$.
\end{definition}
The goal of the levels is to gradually increase difficulty of the learning task while guiding the agent at each level in a way that is similar to curriculum learning \citep{curriculum_learning}. In particular, learning longer timescale option templates typically precedes learning shorter ones.

Extending our above feasibility assumption, we additionally assume that for neighboring environment levels, option templates in one level can be faithfully captured by the policies in the next level.
\begin{assumption}[\textbf{Realizability}]
For any option template
$a_o \in \mathcal{A}_{\optionO}^l$
at level $l$, given by $(\optionI, \optionT, P)$, there is a policy $\pi^{a_o}: \mathcal{S} \rightarrow \mathcal{A}_{\optionO}^{l+1}$ at the following level $l+1$ such that for any $s_0 \in \optionI$,  $\mathsf{Tr}^{o}(s_0) \models \optionT$ 
with probability at least $1-\delta$.
\end{assumption}
That is, any option template in the current level is realizable by a policy in the following level.



\begin{algorithm}[t]
\caption{Learning with Option Templates}
\label{alg:uber_learning}
\textbf{Input: } Environments  $[ \mathcal{E}^0, \mathcal{E}^1, \dots , \mathcal{E}^{n-1} ]$

\textbf{Output: } A set of options $\mathcal{D}=\{o^q\mid q\in Q\}$ that provides an implementation of each option template $a_o^q$, where $q\in Q$ indexes the option templates.

\begin{algorithmic}[1]
\STATE Initialize $\mathcal{D} = \{ \}$
\FOR{level $l \in \{ 1, \dots, n \} $ }
\STATE Let $\mathcal{A}_o^{l-1}$ be the set of option templates on level $l-1$
\STATE Build reward functions $\{ \mathfrak{R}_q \mid a_o^q\in\mathcal{A}_o^{l-1}\} $ 
\FOR{$ a_o^q \in \mathcal{A}_o^{l-1}$ }
\STATE $\pi_o^q=$LearnOptionPolicy$(\mathcal{E}^{l}, \mathfrak{R}_q, a_o^q, \mathcal{D})$ 
\STATE $o^q := $  $(a_o^q, \pi_o^q)$ 
\STATE $\mathcal{D} = \mathcal{D} \cup \{o^q\}$ 
\ENDFOR
\ENDFOR
\OUTPUT $\mathcal{D}$ 
\end{algorithmic}
\end{algorithm}


\subsection{Learning with Option Templates}

Our algorithm for RL with option templates is shown in Algorithm \ref{alg:uber_learning}. Intuitively, at each iteration, it ``flattens'' the option templates used on the previous level $l-1$ based on the ones available at the current level $l$. We give a high-level overview of this algorithm, and provide details below.
\begin{wrapfigure}{r}{0.35\textwidth}
\begin{center}
\includegraphics[width=5cm, height=2.5cm]{Figures/sticky_mittens_learning.png}
\end{center}
\caption{Visualization of learning with option templates.}
\label{fig:sticky-mittens-comp}
\end{wrapfigure}

At each level $l$, we first design reward functions $\mathfrak{R}_q$ for each option template $a_o^q\in\mathcal{A}_o^{l-1}$ (Line 4); this reward function is later used to learn a policy $\pi_o^q$ implementing $a_o^q$.
For the base case $l=1$, we take the reward function $\mathfrak{R}_q$ to be the reward function for the original environment $\mathcal{E}$;
thus, learning the policy for the option-template at this level amounts to accomplishing the goals of $\mathcal{E}$ using the (unique) option template $a_o^q\in\mathcal{A}_o^0$. For subsequent iterations $l>1$, $\mathfrak{R}_q$ encodes the goal of achieving the termination condition of $a_o^q$,
based on its termination condition (Line 4).

Given $\mathfrak{R}_q$, our algorithm learns a policy that maximizes $\mathfrak{R}_q$ using the options available at the current level $l$ (Line 6). For $l=1$, we assume there is a single option template $\mathcal{A}_o^0=\{a_o^q\}$; the corresponding policy $\pi_o^q$ aims to achieve the goal in the original environment $\mathcal{E}$, so we refer to the resulting option $o^q=(a_o^q,\pi_o^q)$ as the \emph{top-level option}. For $l>1$, $\pi_o^q$ implements an option template $a_o^q\in\mathcal{A}_o^{l-1}$ at level $l-1$ using the option templates available at the current level $l$. Importantly, this process leverages policies learned so far to generate initial states from which to learn $\pi_o^q$. Once we have learned $\pi_o^q$, we add the resulting option $o^q=(a_o^q,\pi_o^q)$ to $\mathcal{D}$.



\begin{algorithm}[t]
\caption{Learn Option Policy}
\label{alg:guided_learning}
\textbf{Input: } Environment  $ \mathcal{E}$, Reward Function $\mathfrak{R}$, Option template $a_o=(I,T,P)$, Set $\mathcal{D}$ of options \\
\textbf{Parameter: } Threshold $\delta$, Max Episodes $L$ \\
\textbf{Output: } Policy $\pi_o$ as an implementation of $a_o$

\begin{algorithmic}[1]
\STATE Initialize policy $\pi_o$
\FOR { episode $= 1, \dots, L$ }
\STATE \textit{ExecutionStack} $= [ ]$
\STATE $o$ $\leftarrow$ Top-level option from $\mathcal{D}$ (or $a_o$ if $\mathcal{D}=\varnothing$)
\STATE Push $o$ onto \textit{ExecutionStack}
\STATE Sample initial state $s\sim I$
\WHILE {not done}
\STATE $o\leftarrow$ Pull option from \textit{ExecutionStack} \\
\STATE $o'\leftarrow\pi_{o}(s)$
\IF{IsOption$(o', a_o)$}
\STATE $(\pi_o, s)\leftarrow$ StepAndTrain$(\mathcal{E},\mathfrak{R},\pi_o,s)$
\ELSIF {$\neg$HasImplementation$(o',\mathcal{D})$ } 
\STATE $s\gets$ Teleport$(o',s)$
\ELSE
\STATE Push $o'$ to \textit{ExecutionStack} 
\ENDIF
\ENDWHILE
\STATE Exit loop if AvgReward $\ge1-\delta$
\ENDFOR
\OUTPUT $\pi_o$
\end{algorithmic}
\end{algorithm}



\textbf{Reward function construction.}
Recall that the termination condition for an option starting at state $s_0$ is $\optionT(s_0, k^*) = \mathbf{F}_{o}(s_{k}) \vee (k > k^*)$. The goal of training $\pi_o^q$ is to satisfy this condition with high probability.
Hence, when training policy $\pi_o^q$ for option $a_o^q$, we choose the reward function $\mathfrak{R}_q$ 
to be $\mathbf{F}_{o}$, and additionally restrict the length of each episode to $k^*$ time-steps.

\textbf{Learning option policies.} Next, we describe LearnOptionPolicy, which Algorithm \ref{alg:guided_learning} uses to learn a policy for option template $a_o^q$. For simplicity, we denote the current environment by $\mathcal{E}$, the current reward function by $\mathfrak{R}$,
the option template by $a_o$,
and the target policy by $\pi_o$. The goal of $\pi_o$ is to achieve the termination condition $T$ for $a_o=(I,T,P)$ from initial states $s\in I$. 

One challenge is sampling an initial state $s\in I$ from which to train $\pi_o$. To do so, this subroutine leverages access to the previously learned options $\mathcal{D}$; it uses options in $\mathcal{D}$ until it arrives at a state $s\in I$ where $a_o$ is called.

In more detail, it samples $s$ by executing the top-level option in $\mathcal{D}$ until it reaches a state where $a_o$ is called. In general, executing an option $o$ either relies on executing its policy $\pi_o$ in $\mathcal{D}$ if it exists, or by executing its ``teleport'' functionality. Our algorithm keeps track of the execution of options for which $\pi_o$ exists using a stack, which is initialized with the top-level option (Line 3-5). Then, while executing the current option $o$, it obtains the next option $o'$ to execute, which is processed in one of three ways:
\begin{itemize}
\item If $o'$ is the option for $a_o$ (i.e., it has a matching initial state, termination condition, and a current policy $\tilde \pi_o$, checked by IsOption on Line 10), then it takes steps to train $\pi_o$ (Line 11); as described belowgm.
\item If $o'$ does not have an implementation (checked by HasImplementation on Line 12), then it teleports---i.e., we sample $s\sim P$ (Line 13).
\item Otherwise, $o'$ has an implementation, so it pushes $o'$ onto the stack (Line 15).
\end{itemize}



In general, $o'$ will have an implementation if it is on a level smaller than $l-1$ (since these were learned on previous iterations of Algorithm~\ref{alg:uber_learning}), and will not have an implementation if it is on level $l$; if it is on level $l-1$, then it may or may not have an implementation depending on the order in which policies are learned. This structure is visualized in Figure~\ref{fig:sticky-mittens-comp}.

\begin{figure*}[t!]
    \begin{subfigure}{0.29\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/craft_env_labels.png}
        \caption{Visualization of craft environment for the \textit{get gem} task: The agent (red square) uses the axe in its inventory to break the stone and retrieve the gem.}
        \label{fig:craft}
    \end{subfigure} \hfill 
    \begin{subfigure}{0.29\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/fetch_4/2_midway_v2.png}
        \caption{Visualization of fetch and stack environment: Each block has to be placed at the location represented by the color-coded sphere.}
        \label{fig:fetch}
    \end{subfigure} \hfill 
    \begin{subfigure}{0.375\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/football_env_start_plus.png}
        \caption{Visualization of the Google football environment: The agents learn to use 11 players of the left team and score goals.}
        \label{fig:gfootball}
    \end{subfigure}
    \caption{Craft, Fetch and GFootball environments.}
    \label{fig:env_pictures}
\end{figure*}

Finally, once we are at a state $s$ where $a_o$ is called, the subroutine $StepAndTrain$ takes control and trains $\pi_o$ using a standard reinforcement learning algorithm---i.e., by collecting rewards from $s$ and taking a policy gradient step once it reaches a terminal state or hits the timeout of $k^*$ steps. Then, the current episode continues from the state reached.

Once the current episode reaches a final state, then the algorithm continues to the next episode. This process continues until the average reward of $\pi_o$ exceeds a threshold $1-\delta$, or until a maximum number of episodes $L$ is reached. 


